A continuous multiphase model for liquid metal batteries

Liquid metal batteries (LMBs) are a promising alternative for large-scale stationary energy storage for renewable applications. Using high-abundance electrode materials such as Sodium and Zinc is highly desirable due to their low cost and excellent cell potential. LMBs undergo multiple complex mass transport dynamics and as a result, their operation limits and other critical parameters are not fully understood yet. In this work, a multiphase numerical model was developed to resolve electrode and electrolyte components in 1D and simulate the discharge process of a Na-Zn battery including the interfacial displacement of the molten metal electrodes. The variation in electrolyte composition was predicted throughout the process, including the species distribution and its effect on the cell conductivity and capacity. Volume change and species redistribution were found to be important in predicting the maximum theoretical capacity of the cell when neglecting convective phenomena.

==> archive/archive_old_results.tex <==

After applying a current to the system, we can observe changes in the phase configuration as shown in Figure \ref{fig:profiles} oriented vertically. Here we observe how during the discharge process modelled, the Na interface advances while making way for more electrolyte expansion. At the same time, it is possible to see the deposition of Zn on the right side of the figures. Due to the neglection of gravitational convection, it is possible to see the accumulation of a layer of  $\mbox{Na}^+$ and  $\mbox{Cl}^-$ where the new metallic Zn is deposited. Overall, it can be seen that the $\mbox{Zn}^{+2}$ composition diminishes until depletion.

\begin{figure}[hp]
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/diagram_multi1.png}
    \caption{Diagrams showing the cell in different colours for Na, Cl and Zn ion at different stages in time from top to bottom.}
    \label{fig:profiles}
\end{figure}

In Figure \ref{fig:currents} we show the system composition map at different times after initialization, presented for different currents and at times after the same amount of current has passed. It is possible to observe the interface advancement of the $\text{Na}^+$ is similar, but the composition distribution is different for each value of $J_0$, showing smoother gradients for lower currents and more abrupt ones for higher ones. In the last row, it is possible to observe that the $\mbox{Zn}^{+2}$ has broken contact with the Na interface for the same interface displacement since higher currents lead to more migration-dominated transport inside the electrolyte layer. Overall, this illustrates how the attenuation induced by the diffusion transport in the electrolyte is important to determine the current range at which a certain composition can be attained.   

\begin{figure}[hp]
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/diagram_multi2.png}
    \caption{Area plots showing the volume component composition against its location along the cell. The left column shows all the states after the charge of approximately 1388.88 $\text{Ah/m}^2$ has passed through the system, and the right column shows the same system after 2777.77 $\text{Ah/m}^2$  }
    \label{fig:currents}
\end{figure}

The integrated compositions for the whole system over time are shown in Figure \ref{fig:timeseriesa} and Figure \ref{timeseriesb}, where similarly we show different current intensities against the composition of each system component over time. It can be clearly seen that the electrolyte layer shown (in dashed lines) grows over time at a higher rate as the current is increased. and it can be seen how the $\text{Na}$ layer is eroded while the Zn layer grows, although at different rates given their difference in density. The $\text{Cl}^-$ accumulation appears to grow as a result of the additional expansion of the electrolyte layer and the change in ratios between the other components. 

In the lower row of Figure \ref{fig:timeseries}, we can observe the re-scaled ion compositions adjusted for the molten salt expansion, where we can see how the exchange of $\mbox{Na}^+$ for $\mbox{Zn}^{+2}$ takes place. and it can be seen how at higher currents the rate of exchange appears to be higher. At the highest current, the change appears to be less linear. This can be explained 
by due  depletion and reduced availability of $\mbox{Zn}^{+2}$ at the interface.

\begin{figure}[hp]
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/diagram_mult3a.png}
    \caption{Average compositions over time for each component for different current densities.}
    \label{fig:timeseriesa}
\end{figure}
\begin{figure}[hp]
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/diagram_mult3b.png}
    \caption{Average compositions over time for each component for different current densities, re-scaled to be relative to the total electrolyte volume.}
    \label{fig:timeseriesb}
\end{figure}
In Figure \ref{fig:ohmiclosses}, the total ohmic losses over the whole domain are calculated for each of the currents analyzed. It can be observed that initially, all systems undergo a diminishment in power loss. This is due to the reduced voltage across the cell caused by the initial polarization, given that the boundary current is fixed. This is followed by a monotonic increase in the potential, leading to higher ohmic losses. The reason for this is that the electrolyte layer is getting thicker over time, and given the difference in resistivity in the electrolyte, the total losses increase. 


\begin{figure}[hp]
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/diagram_multi4.png}
    \caption{Ohmic losses over the whole domain for different current densities, a) 500 $A/m^2$, b) 1000 $A/m^2$ c) 2000 $A/m^2$ d) 5000 $A/m^2$}
    \label{fig:ohmiclosses}
\end{figure}

==> figures/Figures.tex <==




==> supplementary_information.tex <==
\section{Supplementary information}
\subsection{Grid sensitivity and mass conservation}
For the purpose of verifying grid convergence, tests were carried out with mesh sizes of 100, 200, 500, 1000, 2000, and 5000 cells. The dimensions and initial conditions of the system are the same as described in the main text. A sample case imposing a constant voltage in charge mode was prepared and repeated with a constant time-step. The total charge time for each case was recorded and compared for each case as shown in Figure \ref{sensitivity_chargeTime}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures_new/SensitivityAnalysis/Fig1.pdf}
    \caption{Recorded charge time for different grids.}
    \label{sensitivity_chargeTime}
\end{figure}

No more significant changes are observed past the 500 cells case, with only minor differences when increasing the resolution further.

For additional confirmation, the final average concentration of each of the components ($ \bar{c}_{i,f}$) is shown in Figure \ref{sensitivity_composition}. The average concentration is presented normalized with its corresponding initial conditions ($\bar{c}_{i,0}$). Although there are differences between cases, these are very minor already at the 1000-cell grid size. With these two criteria, it was decided to use 1000 cells for all the calculations presented in the main text. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures_new/SensitivityAnalysis/Fig2.pdf}
    \caption{Final average concentration for each grid, relative to the initial concentration.}
    \label{sensitivity_composition}
\end{figure}






